MotifPiece: A Data-Driven Approach for Effective Motif Extraction and Molecular Representation Learning

Motif extraction is an important task in motif based molecular representation learning. Previously, machine learning approaches employing either rule-based or string-based techniques to extract motifs. Rule-based approaches may extract motifs that aren't frequent or prevalent within the molecular data, which can lead to an incomplete understanding of essential structural patterns in molecules. String-based methods often lose the topological information inherent in molecules. This can be a significant drawback because topology plays a vital role in defining the spatial arrangement and connectivity of atoms within a molecule, which can be critical for understanding its properties and behavior. In this paper, we develop a data-driven motif extraction technique known as MotifPiece, which employs statistical measures to define motifs. To comprehensively evaluate the effectiveness of MotifPiece, we introduce a heterogeneous learning module. Our model shows an improvement compared to previously reported models. Additionally, we demonstrate that its performance can be further enhanced in two ways: first, by incorporating more data to aid in generating a richer motif vocabulary, and second, by merging multiple datasets that share enough motifs, allowing for cross-dataset learning.

==> Sections/RO1.tex <==

\subsection*{Research Objective 1: Data-Driven Motif Identification and Decomposition}\label{sec:RO1}
\vspace{-6pt}

Motifs, which inherently correlate with molecular properties \cite{debnath1991structure}, significantly influence the performance of molecular graph learning models. Integrating motifs into graph learning requires motif identification and decomposition from molecules.
\textit{Motif identification} refers to recognizing motifs from molecules based on structural or chemical properties. The recognized motifs form a motif vocabulary. On the other hand, \textit{motif decomposition} involves breaking down a given molecule into motifs leveraging the motif vocabulary established during the identification stage.

However, substantial challenges exist in motif identification and decomposition.
1)~The challenge in identifying motifs arises from the lack of an adaptable motif-recognizing method in molecular science. Currently, motif identification methods~\cite{jin2018junction, yu2022molecular, bouritsas2022improving} are either rule-based or string-based. The resulting motifs either lack adaptability or lose chemical semantics, limiting the capability of motif-based molecular graph learning.
% Rule-based methods \cite{jin2018junction, yu2022molecular, bouritsas2022improving} take advantage of pre-defined rules to identify motifs from molecules. The resulting motifs face challenges adapting to various molecular datasets and tasks. The lack of adaptability limits the capability of motif-based molecular graph learning. On the other hand, string-based methods treat molecules as strings and apply text-mining algorithms to identify frequent string patterns. While these methods are beneficial for their adaptability to molecular data, it comes with a key downside of possibly losing chemical semantics. {\color{red} remove related work related parts}
2) The challenge in motif decomposition emerges from the typical representation of motifs in graph format. The decomposition process involves recognizing motifs or subgraphs from the molecular graph and subsequently disassembling the molecular graph into recognized motifs. Recognition of motifs can be viewed as a subgraph isomorphism problem, which verifies the existence of a subgraph within a larger graph. This is a known NP-complete problem, entailing significant computational costs, especially when handling large molecules. 

These challenges motivate the advance of motif identification and decomposition methods. This research objective addresses a key question: \textit{how to effectively recognize data-specific motifs?} 

\noindent\textbf{Current state of the art}: The motif identification methods used by existing motif-based GNNs can be divided into three categories.
1) Ring and bonded pairs (R\&B). Methods~\cite{jin2018junction, yu2022molecular, bouritsas2022improving} in this category recognize simple rings and bonded pairs as motifs.
2) Molecule decomposition. In this category, methods recognize motifs through molecule breakdown. These methods initially establish a catalog of target bonds, either through domain-specific knowledge, such as the ``breakable bonds'' used by RECAP \cite{zhang2021motif} and BRICS \cite{zang2023hierarchical,jiang2023pharmacophoric}, or through hand-crafted rules, like ``bridge bonds'' \cite{jin2020hierarchical}. The algorithms remove these target bonds from the molecules and use the consequent molecular fragments as motifs. 
3) Molecule tokenization. Certain methods~\cite{fang2023single,kuenneth2023polybert} leverage the string representations of molecules, such as SMILES, and directly apply the WordPiece algorithm from the NLP domain. The resulting strings within the constructed vocabulary are regarded as motifs. While these motif strings are adaptive to molecular data, treating molecules purely as strings could introduce problems such as the loss of chemical semantics.

\begin{wraptable}{r}{0.48\linewidth}
\vspace{-12pt}
\caption{Results of using different motif identification methods on MoleculeNet datasets~\cite{wu2018moleculenet}.}
\scriptsize
\vspace{-10pt}
\label{table:ro1}
\begin{tabularx}{\linewidth}{l|YYcc}\hline
        & BBBP           & SIDER          & CLINTOX    & TOX21 \\\hline
BRICS   & 66.03          & 59.19          & 86.52      & \textit{75.32}\\
Bridge  & 63.93          & 58.23          & \textit{86.96}      & 73.89\\
R\&B    & \textit{69.82} & \textit{59.98} & 84.81           & 75.03\\ \hline
New approach  & \textbf{71.14} & \textbf{61.52}   & \textbf{87.69} & \textbf{75.39}\\\hline
\end{tabularx}
\vspace{-10pt}
\end{wraptable}
\noindent\textbf{Preliminary results}:
In our prior work~\cite{yu2022molecular}, we incorporated motifs explicitly into molecular graph learning. We constructed a heterogeneous graph that combined both molecules and associated motifs. The use of GNN on this graph yielded robust performance, highlighting the value of integrating motifs into graph learning. Upon this, we are keen to dive deeper into the role that these identified motifs play. We hypothesize that the method for identifying motifs should be tailored to the specific task. To validate this, we applied several motif identification approaches and incorporated the resulting motifs into our original model. The results are summarized in Table~\ref{table:ro1} showing that no single strategy was universally successful across all tasks. This comparison results motivate the development of data-specific motif identification methods.

To achieve this, we propose a data-driven approach for adaptive motif vocabulary construction and motif decomposition. This approach involves tackling the following open tasks.

\noindent\textbf{\labelText{Task 1.1}{Task:1.1}: Data-driven motif vocabulary construction:}
This task aims to construct a motif vocabulary based on molecular data. We propose a data-driven approach, which applies statistical measures to define motifs. The proposed approach will employ a bottom-up algorithm that starts from simpler motifs (bonded pairs) and progressively assembles more complex ones.

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-20pt}
    \begin{minipage}{\linewidth}
    \begin{algorithm}[H]
        \scriptsize
        \caption{Data-driven motif vocabulary construction}
        \label{alg:motif-defining}
     \begin{algorithmic}
        \STATE {\bfseries Input:} Molecules $\mathcal{G} = \{G_1, \dots, G_n\}$, vocabulary size $V$
        % , and frequency threshold $s$
        \STATE {\bfseries Output:} Motif vocabulary $\mathcal{M}$.
        \STATE {\bfseries Initialization:} Motif vocabulary $\mathcal{M}$ with distinct bonded pairs in $\mathcal{G}$. Motif lists $\{L_1, \dots, L_n\}$ with $L_i$ containing distinct bonded pairs in $G_i$.
        \WHILE{$|\mathcal{M}| < V$}
        \FOR{$G_i$ in $\mathcal{G}$}
            \STATE Enumerate connectable motif pairs based on ${L}_i$.
            \STATE Connect each motif pair to a motif candidate, leading to a candidate set $C_i$.
        \ENDFOR
        \STATE Construct a candidate list $\mathcal{C} = C_1 \cup C_2 \cup\cdots\cup C_n$.
        \STATE Count frequency $d_i$ of each candidate $c_i \in \mathcal{C}$.
        \STATE Select the candidate $c_h$ with the highest frequency.
        % \IF{$d_h < s$}
        % \STATE Exit while.
        % \ENDIF
        \STATE Define $c_h$ as motif and add $c_h$ into $\mathcal{M}$.
        \STATE Update motif lists of molecules 
        % \FOR{molecule $G_i$ in $\mathcal{G}$}
        %     \IF{$c_h$ in $C_i$}
        %         \STATE Add $c_h$ to $L_i$
        %         \STATE Remove two motifs that construct $c_h$ from $L_i$
        %     \ENDIF
        % \ENDFOR
        \ENDWHILE
     \end{algorithmic}
     \end{algorithm}
    \end{minipage}
    \vspace{-12pt}
\end{wrapfigure}
In the initialization stage, we will construct a \textit{motif vocabulary} to store recognized motifs.
% By considering bonded pairs (a bond along with the two atoms it connects) as basic motifs, 
The algorithm will initially add all distinct bonded pairs (a bond along with the two atoms it connects) to the vocabulary. Alongside, an \textit{active motif list} for each molecule will be maintained and initialized using the distinct bonded pairs within the molecule. The active motif lists will be updated as the algorithm iterates by replacing simpler motifs with more complex ones.

Upon initialization, the algorithm will enter a phase of iteration, wherein a new motif will be added to the vocabulary in each cycle. The steps will be as follows: 1) Motif candidate enumeration: Each molecule will enumerate pairs of connectable motifs from its active motif list. A motif pair is considered connectable if they share the same atoms in the original molecule. Each pair will then be linked into a motif candidate, forming a larger subgraph containing all the atoms and bonds from both motifs. The unique motif candidates across all molecules will form the motif candidate list. 2) Candidate frequency counting: For each motif candidate, we will calculate its occurrence frequency across all molecules. 3) New motif recognition: If the frequency of the most common motif candidate surpasses a threshold, it will be added to the motif vocabulary as a new motif. 4) Active motif list update: The new motif will be added to the active motif lists in which it appears. Also, the motifs that formed this new motif will be removed from active motif lists.
% Following initialization, the algorithm enters an iterative phase. A new motif is added to the vocabulary in each iteration by the following steps. 1) Enumerate motif candidates: Each molecule will enumerate pairs of connectable motifs from its active motif list. Connectable motif pairs as those sharing the same atoms in the original molecule. Each connectable pair is then connected into a motif candidate. Given that motifs are subgraphs of the original molecular graph, the two motifs or subgraphs are connected through their common atoms. They connect to a motif candidate or another subgraph that includes all the atoms and bonds from both motifs. The distinct motif candidates across all molecules construct the \textit{motif candidate list}. 2) Count candidate frequency: For each motif candidate in the candidate list, we calculate its frequency in all molecules. 3) Recognize new motif: the most frequently occurring candidate will be added to the motif vocabulary as the new motif if its frequency is higher than a predetermined threshold. This ensures that the most common patterns across the molecules are captured. 4) Update individual active motif list: the newly recognized motif is added to the active motif lists of molecules it presents, while the motifs that form the new one are removed.
% The algorithm iterates this way until the vocabulary has reached a predetermined size or no motif is newly defined. Ultimately, the algorithm will yield a motif vocabulary containing data-specific motifs recognized from the given molecular data. Algorithm~\ref{alg:motif-defining} describes this process. The basic ideas were tested using the same setting in the preliminary results. From promising results in Table~\ref{table:ro1} primarily demonstrate the capability of data-driven motif identification. The PI will investigate the proposed methods in general molecular graph learning settings.
The algorithm will continue until the motif vocabulary reaches a pre-specified size or no new motifs are identified. Eventually, a motif vocabulary of motifs unique to the given molecular data will be generated. This process is described in Algorithm~\ref{alg:motif-defining}. Preliminary tests have been conducted with results shown in Table~\ref{table:ro1}, highlighting the potential of data-driven motif identification. The PI will explore these methods in broader molecular learning contexts.

\noindent\textbf{\labelText{Task 1.2}{Task:1.2}: Data-driven motif decomposition.}
This task aims to design an algorithm that can decompose a given molecule into motifs, using a motif vocabulary as built in~\ref{Task:1.1}.
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \vspace{-18pt}
%     \begin{minipage}{\linewidth}
%     \begin{algorithm}[H]
%         \scriptsize
%         \caption{Data-driven motif decomposition}
%         \label{alg:motif-identification}
%      \begin{algorithmic}
%         \STATE {\bfseries Input:} Molecular graph $G$ and a motif vocabulary $\mathcal{M}$.
%         \STATE {\bfseries Output:} Motif list $L$.
%         \STATE {\bfseries Initialization:} Motif list $L$ containing bonded pairs in $G$.
%         \WHILE{\TRUE}
%             \STATE Enumerate connectable motif pairs based on $\mathcal{L}$.
%             \STATE Connect each motif pair to a candidate using atoms and bonds from both motifs, leading to a candidate set $C$.
%         \STATE Select the candidate $c_h \in C$ with the highest complexity and $c_h \in \mathcal{M}$.
%         \IF{no candidate selected}
%         \STATE Exit while.
%         \ENDIF
%         \STATE Add $c_h$ to $L$
%         \STATE Remove two motifs that construct $c_h$ from $L$
%         \ENDWHILE
%      \end{algorithmic}
%      \end{algorithm}
%     \end{minipage}
%     \vspace{-12pt}
% \end{wrapfigure}
At the start of the process, a motif vocabulary $\mathcal{M}$ is given. We will create a motif list to store motifs identified from the molecule. This motif list will be initialized with its bonded pairs, serving as the primary motifs. Note that the same motif's multiple instances will all be in the list.
The algorithm will enter an iterative phase to gradually recognize more complex motifs. Each iteration will include the following steps:
1) Enumerate motif candidates: the algorithm will create motif candidates by enumerating pairs of connectable motifs from the current motif list. Each connectable pair is integrated into a more complex motif candidate.
2) Identify a motif: Among the motif candidates, the most complex one (in terms of the number of nodes and edges) that appears in the vocabulary will be selected as the new motif. Complexity is used as a selection criterion to ensure the most representative patterns are captured.
3) Update motif list: The new motif will be added, and the ones used to form it will be removed.
This iterative process will continue until no further motifs can be found. Eventually, the algorithm will output a list of motifs decomposed from the molecule.
% This process is detailed in Algorithm~\ref{alg:motif-identification}.

\noindent\textbf{Time complexity analysis.}
Our proposed algorithm begins with a motif list composed of basic bonded pairs. In each iteration, the size of this list reduces by one, and in the worst-case scenario, the algorithm runs for $E$ iterations, where $E$ is the total number of bonds. However, within each iteration, we enumerate $6N$ potential motif pairs at most, with $N$ being the number of atoms. Given the maximum degree of $4$ for an atom in a molecular graph, up to $6$ motif pairs can be produced when an atom acts as a shared node. All the other operations are linear with the size of motif pairs, except for checking the motif candidate's existence in the motif vocabulary. As the following task explains, this step has a time complexity of $O(N+E)$. Consequently, the overall time complexity of the algorithm is $O((N+E)E)$.

% The initial motif list comprises basic bonded pairs in the proposed algorithm. The algorithm iterates and reduces the motif list size by one in each iteration. It will execute a maximum of $E$ times in the worst-case scenario, where $E$ is the number of bonds. However, within each iteration, there are at most $6N$ potential motif pairs to enumerate, where $N$ is the number of atoms. Each atom in a molecular graph can have a maximum degree of $4$, producing up to $6$ motif pairs by acting as the shared node. The remaining operations all show a linear relationship with the size of the motif pairs, except for the motif candidate's existence check within the motif vocabulary. As detailed in the next task, our proposed approach can achieve a time complexity of $O(N+E)$ for this step. As a result, the inner loop's time complexity becomes $O(N+E)$, bringing the overall time complexity to $O((N+E)E)$.

\noindent\textbf{\labelText{Task 1.3}{Task:1.3}: String-based molecular graph matching.}
This task aims to solve the efficiency challenges faced by motif identification methods. 
% To this end, the PI proposed a linear molecular graph-matching algorithm.
% As mentioned previously, most motif identification methods suffer from efficiency challenges for recognizing motifs from large and complex molecules, which is not currently known to be solvable in polynomial time. This challenge also applies to our proposed algorithms in \ref{Task:1.1} and \ref{Task:1.2}. Solving this challenge will not only enable broader application scenarios of the proposed methods But also help with other motif identification methods. Thus, this task aims to develop an efficient molecular graph-matching algorithm.
We propose a string-based approach for molecular graph matching with linear time complexity. The approach will use the unique properties of molecular graphs, such as specific node identities, unique edges, and predictable structures governed by chemical rules. It will consist of two steps. 1) Molecular subgraph canonicalization: We will convert the molecular subgraphs into canonical strings using molecular canonicalization methods~\cite{schneider2015get}. This will ensure a unique SMILES string for each molecule subgraph, irrespective of atom order or other variations. 2) String matching: If two strings are identical, we will consider the molecular subgraphs to be the same. Our string-based approach combines the efficiency of graph traversal with string-matching algorithms, providing an efficient solution for molecular graph matching.

% We propose a string-based molecular graph-matching approach instead of working with graph format. Unlike regular graphs, molecular graphs can be converted into strings due to their inherent properties of specific node identities, uniqueness of edges, and predictable structure based on chemical rules. As such, our approach proceeds by the following two steps. 1) Molecular canonicalization. Using a molecular canonicalization method, we first transform the given molecular subgraphs into canonical SMILES strings. This process ensures the one-to-one correspondence between a molecule and its canonical SMILES string, regardless of the order of atom input or other variations. 2) String matching. Once the molecules are represented as SMILES strings, we directly compare them. The molecular subgraphs will be considered identical if the two strings are identical. Overall, the string-based molecular graph-matching approach leverages the theoretical efficiency of graph traversal and string-matching algorithms to provide a more efficient solution for molecular subgraph matching.

\noindent\textbf{Time complexity analysis.}
This algorithm comprises two main operations: the conversion of molecules into SMILES strings and string comparison. Generating canonical SMILES strings from molecules is fundamentally a depth-first search graph traversal procedure, which carries a linear computational complexity $O(N+E)$. Similarly, the time complexity for comparing two strings is also linear. Consequently, the overall time complexity for this graph-matching algorithm is linear.

% {\color{red} can change to extension to 3d motifs}
\noindent\textbf{\labelText{Task 1.4}{Task:1.4}: Data-driven 3D motif identification.}
In molecular science, a 3D motif is a specific grouping of atoms frequently recurs in 3-dimensional space. Even with the same 2D structures, different 3D layouts can produce substantial differences in properties like reactivity, stability, and binding affinity~\cite{bickelhaupt2003case}. For example, staggered ethane is more stable than eclipsed ethane, despite the same 2D structure (C2H6). Figure~\ref{fig:3dmotif} illustrates an example of 3D motifs. It is critical to identify 3D motifs for molecular graph learning.

% In molecular science, a 3D motif refers to a recurrent specific arrangement of atoms in three-dimensional space.
% Unlike 2D motifs, which only account for chemical connectivity, 3D motifs incorporate the spatial relationships between atoms, including angles between bonds and distances between atoms. 
% Notably, identical 2D motifs can show distinct 3D layouts, leading to significantly different properties such as reactivity, stability, and binding affinity. For instance, the stability of staggered ethane (C2H6) is higher than that of eclipsed ethane (C2H6), despite their identical 2D representations. Hence, identifying 3D motifs is crucial for 3D molecular graph learning.

\begin{wrapfigure}{r}{0.28\textwidth}
    \vspace{-22pt}
    \includegraphics[width=\linewidth]{FIG/3Dmotif.pdf}
    \vspace{-20pt}
    \caption{3D motifs sharing the same 2D motif.}
    \vspace{-12pt}
    \label{fig:3dmotif}
\end{wrapfigure}
In this task, the PI aims to enhance the proposed motif identification algorithms to handle 3D scenarios. The procedure is as follows:
1) Constructing 3D motif vocabulary: We will use the 2D motifs identified in Task~\ref{Task:1.1}. For each 2D motif, we will detect common 3D motifs. We will generate a unique fingerprint for every 3D instance of the same 2D motif using 3D molecular fingerprint methods. Direct frequency matching of these 3D fingerprints is challenging due to factors like measurement errors. To handle this, we will use an agglomerative clustering algorithm. It will merge the closest pairs of 3D motif instances iteratively until the smallest distance surpasses a threshold. We will treat the resulting clusters' centers as 3D motifs.
2) Decomposing a molecule: We will apply a 2D motif decomposition algorithm to a molecule, producing a set of 2D motifs. For each 2D motif instance, we will create its 3D fingerprint. We will assign it to the nearest 3D motif in the vocabulary.

% In this task, the PI will extend the proposed motif identification algorithms to accommodate 3D scenarios through the following steps:
% 1) 3D motif vocabulary construction: We initially utilize 2D motifs identified from~\ref{Task:1.1} to mitigate computational costs. For each 2D motif, we'll recognize its corresponding frequently-occurring 3D motifs. For each instance of a 2D motif in the molecular data, we'll generate a unique fingerprint using 3D molecular fingerprint methods. Given the challenge of directly matching the frequency of these 3D fingerprints caused by factors like measurement errors, we'll use an agglomerative clustering algorithm. This algorithm will iteratively merge the nearest pair of 3D motif instances until the minimum distance exceeds a predefined threshold. The resulting clusters' centers will then be recognized as 3D motifs.
% 2) 3D Motif Decomposition: Adopting a similar approach, we will initially employ a 2D motif decomposition algorithm to a given molecule, resulting in a set of 2D motifs. For each 2D motif, we will then generate its corresponding 3D fingerprint. Subsequently, each instance of a 2D motif will be assigned to its most closely aligned 3D motif in the pre-established 3D motif vocabulary.
